My Mouse, My Rules: Privacy Issues of Behavioral User Profiling via Mouse Tracking

This paper aims to stir debate about a disconcerting privacy issue on web browsing that could easily emerge because of unethical practices and uncontrolled use of technology. We demonstrate how straightforward is to capture behavioral data about the users at scale, by unobtrusively tracking their mouse cursor movements, and predict user's demographics information with reasonable accuracy using five lines of code. Based on our results, we propose an adversarial method to mitigate user profiling techniques that make use of mouse cursor tracking, such as the recurrent neural net we analyze in this paper. We also release our data and a web browser extension that implements our adversarial method, so that others can benefit from this work in practice.

==> Makefile <==
# This Makefile allows to compile the paper in a temp dir, to avoid syncing autogenerated files in Dropbox.

PAPER = main
CURDIR = "$(shell pwd)"
OUTDIR = /tmp/mouse-privacy

all: dirs paper bib
	$(MAKE) paper
	$(MAKE) bib
	$(MAKE) paper
	$(MAKE) paper

dirs:
	mkdir -p $(OUTDIR)

paper: dirs $(wildcard *.tex)
	pdflatex -output-directory $(OUTDIR) $(PAPER).tex

bib: paper
	cd $(OUTDIR); ln -sf $(CURDIR)/acmart.bst .; \
	              ln -sf $(CURDIR)/refs.bib .; \
	              bibtex $(PAPER).aux; \
	              cd -

clean: dirs
	cd $(OUTDIR); rm -f $(PAPER).out $(PAPER).aux $(PAPER).log $(PAPER).blg $(PAPER).bbl \
	                    $(PAPER).toc $(PAPER).spl $(PAPER).tpt $(PAPER).synctex.gz $(PAPER).bcf $(PAPER).run.xml}; \
	              cd -

